Boundedness of varieties of Fano type with alpha-invariants and volumes bounded below

We show that fixed dimensional klt weak Fano pairs with alpha-invariants and volumes bounded away from $0$ and the coefficients of the boundaries belong to the set of hyperstandard multiplicities $\Phi(\mathscr{R})$ associated to a fixed finite set $\mathscr{R}$ form a bounded family. We also show $\alpha(X,B)^{d-1}\mathrm{vol}(-(K_X+B))$ are bounded from above for all klt weak Fano pairs $(X,B)$ of a fixed dimension $d$.

==> 5.bdd.tex <==
\section{Towards boundedness of rationally connected klt Calabi--Yau's}\label{section 7}

We have seen so far that rationally connected klt Calabi--Yau $3$-folds
are birationally bounded in Section \ref{sec 3}. By applying results in Section \ref{sec 4}, in a good number of cases, it is actually possible to prove that boundedness holds
under slightly stronger assumptions.

Firstly we show that rationally connected klt Calabi--Yau $3$-folds with mld bounded away from $1$ are  bounded modulo flops.
\begin{thm}\label{t.bdd.mld}
Fix $0<c<1$.
Let $\mathcal{D}$ be the set of varieties $X$ such that
\begin{enumerate}
%\item $X$ is a projective klt $3$-fold
\item $X$ is a rationally connected klt Calabi--Yau $3$-fold, and
\item $0<\mld(X)< c$.
\end{enumerate}
Then $\mathcal{D}$ is   bounded modulo flops. 
\end{thm}

\begin{proof}
Take $X\in \mathcal{D}$. % be a rationally connected Calabi--Yau $3$-fold with $0<\mld(X)\leq c$. %Note that $X$ has worse than canonical singularities, that is, there exists a closed point $p\in X$ such that $\mld_p(X)<1$. 
%By assumption, there exists a constant $c \in (0,1)$ such that $\mld_p(X)<c$.
By \cite[Corollary 1.4.3]{BCHM}, we may take   a birational morphism $\pi \colon Y \to X$ extracting only one exceptional 
divisor $E$ of log discrepancy $a=a(E, X) \in (0, c)$. Then
\[
K_Y+(1-a)E = \pi^\ast K_X.
\]
Also by Global ACC (see Lemma \ref{klt=e-klt}), there exists a constant $\epsilon \in (0,\frac{1}{2})$ such that $X$ is $(2\epsilon)$-lc, and therefore $(Y, (1-a)E)$ is a $(2\epsilon)$-lc log Calabi--Yau pair with $1-a>1-c>0$ and $Y$ rationally connected. 

Now  by Corollary \ref{cor.bdd.lcy3fold}, the pairs $(Y, E)$ are log bounded modulo flops.
%since the coefficients of $\Delta$ can only vary in 
%a finite set. Let us notice that in order to apply said theorem, we would
%need to verify that $Y$ is not of product type, but this is not needed, as noted
%at the end of the paper when the dimension of $Y$ is three. Hence, we will
%substitute the pair $(Y, \Delta)$ with a corresponding pair (isomorphic in
%codimension one) that appears as a fibre of the bounded family constructed in \cite{DCS}.
That is, there are finitely many quasi-projective normal varieties $\mathcal{W}_i$, a reduced divisor $\mathcal{E}_i$ on $\mathcal W_i$, and a projective morphism $\mathcal{W}_i\to S_i$, where $S_i$ is a normal variety of finite type and $\mathcal{E}_i$ does not contain any fiber, such that
for every $(Y, E)$, there is an index $i$, a closed point $s \in S_i$, and a small birational
map $f : {\mathcal{W}_{i,s}} \dashrightarrow Y$
such that $\mathcal{E}_{i,s}=f_*^{-1}E$. We may assume that the set of points $s$ corresponding to such $Y$ is dense in each $S_i$.
We may just consider a fixed index $i$ and ignore the index in the following argument.

For the point $s$ corresponding to $(Y,E)$, $$K_{{\mathcal{W}_s}}+(1-a)f_*^{-1}E\equiv f_*^{-1}(K_Y+(1-a)E)\equiv 0$$ and therefore $({\mathcal{W}_s}, (1-a)f_*^{-1}E)$ is a $(2\epsilon)$-lc log Calabi--Yau pair. % where $\epsilon=\frac{1}{2r}$.
Now consider a log resolution $g: \mathcal{W}'\to \mathcal{W}$ of $(\mathcal{W},\mathcal{E})$ and denote by $\mathcal{E}'$ the strict transform of $\mathcal{E}$ and all the sum of $g$-exceptional reduced divisors on $\mathcal{W}'$. Consider the log canonical pair $(\mathcal{W}',(1-\epsilon)\mathcal{E}')$. 
There exists an open dense set $U\subset S$ such that for the point $s\in U$ corresponding to $(Y,E)$, 
$g_s: \mathcal{W}'_s\to \mathcal{W}_s$ is a log resolution and we can write
$$
K_{\mathcal{W}'_s}+B_s=g_s^*(K_{{\mathcal{W}_s}}+(1-a)f_*^{-1}E)\equiv 0
$$
where the coefficients of $B_s$ are $\leq 1-2\epsilon$ and its support is contained in $\mathcal{E}'_s=\mathcal{E}'|_{{\mathcal{W}'_s}}$. We have
\begin{align*}
{}&(K_{\mathcal{W}'}+(1-\epsilon)\mathcal{E}')|_{{\mathcal{W}'_s}}\\
\equiv {}&K_{\mathcal{W}'_s}+(1-\epsilon)\mathcal{E}'_s\\
\equiv {}&(1-\epsilon)\mathcal{E}'_s-B_s.
\end{align*}
Note that the support of $(1-\epsilon)\mathcal{E}'_s-B_s$ coincides with the support of $\mathcal{E}'_s$ which are precisely the divisors on $\mathcal{W}'_s$ exceptional over $X$. Hence $(K_{\mathcal{W}'}+(1-\epsilon)\mathcal{E}')$ is of Kodaira dimension zero on the fiber $\mathcal{W}'_s$ and we can run a $(K_{\mathcal{W}'}+(1-\epsilon)\mathcal{E}')$-MMP with scaling of an ample divisor over $S$ to get a relative minimal model $\tilde{\mathcal{W}}$ over $S$. Such MMP terminates by \cite[Corollary 2.9, Theorem 2.12]{HX13}. Note that for the point $s\in U$ corresponding to $(Y,E)$, $\mathcal{E}'_s$ is contracted and hence $\tilde{\mathcal{W}}_s$ is isomorphic to $X$ in codimension one. This gives a bounded family modulo flops, over $U$.
Applying Noetherian induction on $S$, the family of all such $X$ is bounded modulo flops.
%As this is a bounded family, by noetherian induction and finiteness of the
%coefficients, there exists $0<\epsilon \ll 1$ such that $(Y, (1+\epsilon)\Delta)$ is 
%klt. But then, using noetherian induction and \cite[Theorem 1.1]{HX13}, there are
%finitely many families that parametrize the minimal models of $(Y, (1+\epsilon)\Delta)$.
%Since the Kodaira dimension of $\Delta$ is $0$, the minimal model of $(Y, (1+\epsilon)\Delta)$
%is isomorphic in codimension $1$ to $X$, which proves the claim.
\end{proof}




%This is the case, for example, if we bound Cartier index of the canonical divisor.
%\iffalse
%\begin{cor}\label{c.bdd.ind}
%Fix $r \in \mathbb{N}_{>0}$.
%Let $\mathcal{D}$ be the set of varieties $X$ such that
%\begin{enumerate}
%\item $X$ is a projective klt $3$-fold
%\item $X$ is a rationally connected klt Calabi--Yau $3$-fold, and
%%\item $rK_X \sim 0$.
%\end{enumerate}
%Then $\mathcal{D}$ is  strongly birationally bounded. % family. %bounded in codimension one. 
%\end{cor}

%\begin{proof}
%Since for any $X \in \mathcal{D}, 
%\; rK_X$ is a Cartier divisor, then set of log discrepancies 
%\[
%\{a(E, X) \; | \; X \in \mathcal{D}, \; E \text{ exceptional over } X \}
%\]
%is contained in $\frac 1{r} \mathbb Z \cap [0,1)$. 

%By \cite[Corollary 1.4.3]{BCHM}, we can take a birational morphism $\pi \colon Y \to X$ extracting precisely all
%the exceptional divisors $E$ over $X$ with log discrepancy $a(E, X) \in (0, 1)$. % -- which exists by \cite[Corollary 1.4.3]{BCHM}.
%We can write
%Let $\Delta$ be the divisor in the formula
%\[
%K_Y+\Delta = \pi^\ast K_X\equiv 0.
%\]
%Since $rK_X$ is Cartier, $(Y, \Delta)$ is $\frac{1}{r}$-lc and the coefficients of $\Delta$ belongs to the finite set $\frac 1{r} \mathbb Z \cap (0,1)$. Moreover, $Y$ is rationally connected and $(Y, \Delta)$ has at worst canonical singularities by the construction, which implies that $K_Y$ is not pseudo-effective and hence $\Delta>0$.
%Therefore, the set of such pairs $(Y, \Delta)$ is log bounded in codimension one by 
%\cite[Theorem 1.3]{DCS} or Corollary \ref{cor.bdd.lcy3fold}.
%since the coefficients of $\Delta$ can only vary in 
%a finite set. Let us notice that in order to apply said theorem, we would
%need to verify that $Y$ is not of product type, but this is not needed, as noted
%at the end of the paper when the dimension of $Y$ is three. Hence, we will
%substitute the pair $(Y, \Delta)$ with a corresponding pair (isomorphic in
%codimension one) that appears as a fibre of the bounded family constructed in \cite{DCS}.
%That is, there is a quasi-projective scheme $\mathcal{W}$, a reduced divisor $\mathcal{E}$ on $\mathcal W$, and a projective morphism $\mathcal{W}\to S$, where $S$ is of finite type and $\mathcal{E}$ does not contain any fiber, such that
%for every $(Y, \Delta)$, there is a closed point $s \in S$ and a small birational
%map $f : {\mathcal{W}_s} \dashrightarrow Y$
%such that $\mathcal{E}_s$ coincides with the support of $f_*^{-1}\Delta$. By noetherian induction, we may assume that $\mathcal{W}$ and $S$ are normal varieties and the set of points $s$ corresponding to such $Y$ is dense in $S$. Also we may assume that $\mathcal{W}$ is $\bQ$-factorial by the construction. In particular, for the point $s$ corresponding to $(Y,\Delta)$, $K_{{\mathcal{W}_s}}+f_*^{-1}\Delta\equiv f_*^{-1}(K_Y+\Delta)\equiv 0$ and therefore $({\mathcal{W}_s}, f_*^{-1}\Delta)$ is a $(2\epsilon)$-lc log Calabi--Yau pair where $\epsilon=\frac{1}{2r}$.

%Now consider a log resolution $g: \mathcal{W}'\to \mathcal{W}$ of $(\mathcal{W},\mathcal{E})$ and denote by $\mathcal{F}$ the exceptional divisors and $\mathcal{E}'$ the strict transform of $\mathcal{E}$. Consider the log canonical pair $(\mathcal{W}',(1-\epsilon)\mathcal{E}'+(1-\epsilon)\mathcal{F})$. 
%There exists an open dense set $U\subset S$ such that for the point $s\in U$ corresponding to $(Y,\Delta)$, 
%$g_s: \mathcal{W}'_s\to \mathcal{W}_s$ is a log resolution and we can write
%$$
%K_{\mathcal{W}'_s}+B_s=g_s^*(K_{{\mathcal{W}_s}}+f_*^{-1}\Delta)\equiv 0
%$$
%where the coefficients of $B_s$ are $\leq 2\epsilon$.
%\begin{align*}
%{}&(K_{\mathcal{W}'}+(1-\epsilon)\mathcal{E}'+(1-\epsilon)\mathcal{F})|_{{\mathcal{W}_s}}\\
%\equiv {}&K_{\mathcal{W}'_s}+(1-\epsilon)\mathcal{E}'|_{{\mathcal{W}'_s}}+(1-\epsilon)\mathcal{F}|_{{\mathcal{W}'_s}}\\
%\equiv {}&(1-\epsilon)\mathcal{E}'|_{{\mathcal{W}'_s}}+(1-\epsilon)\mathcal{F}|_{{\mathcal{W}'_s}}-B_s
%\end{align*}
%Note that the support of $(1-\epsilon)\mathcal{E}'|_{{\mathcal{W}'_s}}+(1-\epsilon)\mathcal{F}|_{{\mathcal{W}'_s}}-B_s$ coincides with the support of $\mathcal{E}'|_{{\mathcal{W}'_s}}+\mathcal{F}|_{{\mathcal{W}'_s}}$ which are precisely the divisors on $\mathcal{W}'_s$ exceptional over $X$. Hence $(K_{\mathcal{W}'}+(1-\epsilon)\mathcal{E}'+(1-\epsilon)\mathcal{F})|_{{\mathcal{W}_s}}$ is of Kodaira dimension zero and we can run a $(K_{\mathcal{W}'}+(1-\epsilon)\mathcal{E}'+(1-\epsilon)\mathcal{F})$-MMP over $S$ to get a relative minimal model $\tilde{\mathcal{W}}$ over $S$ such that  for the point $s\in U$ corresponding to $(Y,\Delta)$, $\mathcal{E}'|_{{\mathcal{W}'_s}}+\mathcal{F}|_{{\mathcal{W}'_s}}$ is contracted and $\tilde{\mathcal{W}}_s$ is isomorphic to $X$ in codimension one. This gives a bounded family over $U$.
%Applying neotherian induction again, all such $X$ is bounded in codimension one.
%As this is a bounded family, by noetherian induction and finiteness of the
%coefficients, there exists $0<\epsilon \ll 1$ such that $(Y, (1+\epsilon)\Delta)$ is 
%klt. But then, using noetherian induction and \cite[Theorem 1.1]{HX13}, there are
%finitely many families that parametrize the minimal models of $(Y, (1+\epsilon)\Delta)$.
%Since the Kodaira dimension of $\Delta$ is $0$, the minimal model of $(Y, (1+\epsilon)\Delta)$
%is isomorphic in codimension $1$ to $X$, which proves the claim.
%\end{proof}
%\fi

As an interesting application, we can show that for rationally connected klt Calabi--Yau $3$-folds,  the boundedness modulo flops is equivalent to the boundedness of global index.

\begin{cor}\label{c.bdd.index}
Let $\mathcal{D}$ be a set of rationally connected klt Calabi--Yau $3$-folds.
Then $\mathcal{D}$ is  bounded modulo flops if and only if
there exists a positive integer $r$ such that $rK_X\sim 0$ for any $X\in \mathcal{D}$.
\end{cor}

\begin{proof}
Assume that $\mathcal{D}$ is bounded modulo flops, then 
there exists a bounded family $\mathcal{D}'$ of normal projective varieties such that for every $X\in \mathcal{D}$, there exists $Y\in\mathcal{D}'$ and a small birational morphism $f: Y\dashrightarrow X$. Moreover, $K_Y$ is $\bQ$-Cartier by the definition. Hence we have $K_Y=f_*^{-1}K_X\sim_\bQ 0$.
Take a common resolution $p:W\to Y$ and $q:W\to X$,
by the Negativity Lemma, we have $p^*K_Y=q^*K_X$ and $Y$ is klt.
Since $\mathcal{D}'$ is bounded, there exists a constant $r \in \mathbb{N}_{>0}$ such that $rK_Y$ is Cartier, which means that $p^*(rK_Y)\sim_\bQ 0$ is a Cartier divisor. Since $W$ is rationally connected, it is simply connected and hence $p^*(rK_Y)\sim 0$. Therefore $rK_X=q_*q^*(rK_X)\sim 0$. This proves the `only if' part.

%by \cite[Prop. 2.5]{HX15} there exists a family $(\mathcal Y , \mathcal F)\to T$
%over a quasi-projective base $T$ such that for any $X_i \in \mathcal{D}$ and 
%any set of divisors $E_{i,j}$ with $j\in I_i$ such that $E_{i,j}$ is exceptional of discrepancy $a(E_{i,j},X_i,B_i)\leq 0$, then there exists $t\in T$ and a morphism $\mu _t : \mathcal Y _t \to X_i$ which extracts precisely the divisors $E_{i,j}$ with $j\in I_i$  such that $K_{\mathcal Y _t}+  \mathcal F _t=\mu _t^*(K_{X_i})$.
%Using noetherian induction and resolving $(\tilde{Y}, \tilde{\mathcal F}) \to (Y, \mathcal F)$, 
%we can assume that the pairs $(Y_t, \mathcal F_t)$ are log smooth over $T$. 
%Applying \cite[Theorem 4.2]{HMX14_b} to the pairs $(\tilde{Y}_t, \tilde{\mathcal F}_t)$, it follows
%that there exists $n \in \mathbb{N}_{>0}$ such that $n(K_{Y_u}+\mathcal{F}_u) \sim 0$ and so
%the same conclusion must hold for any $X \in m\mathcal{D}$.

%If there exists $r \in \mathbb{N}_{>0}$ such that $rK_X\sim 0$ for  any $X\in \mathcal{D}$, then the implication 
If there exists a positive integer $r$ such that $rK_X\sim 0$ for any $X\in \mathcal{D}$, then it is clear that $r\cdot \mld(X)$ is a positive integer.  Since $X$ is rationally connected, $X$ has worse than canonical singularities, that is, $\mld(X)<1$. Therefore $\mld(X)\leq 1-\frac{1}{r}<1-\frac{1}{2r}$. 
The `if' part follows directly from Theorem \ref{t.bdd.mld}.
\end{proof}

As another application, Theorem \ref{t.bdd.mld} relates Conjecture \ref{conj1} to conjectures for minimal log discrepancies. Recall the following deep conjecture regarding the behavior of minimal log discrepancy proposed by Shokurov. 
\begin{conj}[ACC for mld, cf. {\cite[Problem 5]{Sho88}, \cite[Conjecture 4.2]{MR1420223}}]\label{c.mld.strong}
Fix a positive integer $d$ and a DCC set $I \subset [0,1]$. Then the set
\[
\{\mathrm{mld}_{\eta_Z}(X, \Delta) \; \mid \; (X, \Delta) \text{ is lc}, \; \dim X\leq d, \;
Z\subset X, \; \mathrm{coeff}(\Delta) \in I \}
\]
satisfies the ACC. 
\end{conj}

ACC stands for ascending chain condition whilst DCC stands for descending chain condition. 

Here we only need a very weak version of Conjecture \ref{c.mld.strong}.

\begin{conj}[1-Gap conjecture for mld]\label{c.mld}Fix a positive integer $d$.
Then $1$ is not an accumulation point from below for the set
\[
\{\mathrm{mld}(X) \; \mid \; \dim X\leq d\}.
\]
\end{conj}


\begin{cor}\label{t.bdd.cyklt}
Assume that Conjecture \ref{c.mld} holds for rationally connected klt Calabi--Yau $3$-folds. Then the set of  rationally connected klt Calabi--Yau $3$-folds is bounded modulo flops. %
%bounded in codimension one.
\end{cor}

\begin{proof}
Let $X$ be a rationally connected klt Calabi--Yau $3$-fold. Note that $X$ has worse than canonical singularities, that is, $\mld(X)<1$. 
By Conjecture \ref{c.mld}, there exists a constant $c \in (0,1)$ such that $\mld(X)< c$.
Hence the corollary follows directly from Theorem \ref{t.bdd.mld}. 
\end{proof}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Finally we consider  rationally connected klt Calabi--Yau $3$-folds with positive augmented irregularity. For klt Calabi--Yau varieties, Greb, Guenancia, and Kebekus 
proved that there is a decomposition,
after quasi-\'etale covering, that is analogous to the classical
Beauville--Bogomolov decomposition in the smooth case, \cite{MR730926}.

\begin{thm}[{\cite[Theorem B]{ggk}}]\label{t.ggk}
Let $X$ be a klt variety with $K_X\equiv 0$. Then there are
normal projective varieties $A, Z$ and a quasi-\'etale cover
$\gamma \colon A\times Z \to X$ such that 
\begin{enumerate}
\item $A$ is an abelian variety of dimension $\tilde{q}(X)$,
\item $Z$ has canonical singularities, $K_Z\sim 0$ and 
$\tilde{q}(Z)=0$, and
\item there exists a flat K\"ahler form $\omega_A$ on $A$
and a singular Ricci-flat K\"ahler metric $\omega_Z$ on $Z$
such that $\gamma^\ast \omega_H = \mathrm{pr}_1^\ast 
\omega_A + \mathrm{pr}_2^\ast \omega_Z$ and such that
the holonomy group of the corresponding Riemann metric 
on $A \times Z_{reg}$ is connected.
\end{enumerate}
\end{thm}

Here we recall the notion of augmented irregularity. % which plays a fundamental
%role in \cite[Definition 2.6]{MR2587100}.

\begin{definition}[{cf. \cite[Definition 2.20]{ggk}}]\label{d.gen.irr}
Let $X$ be a normal projective variety. The {\it irregularity} of $X$ is defined
as $q(X):= h^1(X, \mathcal{O}_X)$.
The {\it augmented irregularity} of $X$ is defined as $\tilde{q}(X)= \sup \{ q(Y)\; | \;  Y \to X \; \text{quasi-\'etale cover}\} \in \mathbb{N} \cup \{\infty\}$.
\end{definition}

\begin{remark}
When $X$ has rational singularities (as it will be the case
in this section), then $q(X) = q(Z)$ for any $Z \to X$ resolution
of singularities.
\end{remark}

As a consequence of the decomposition for singular Calabi--Yau 
varieties and Theorem \ref{t.bdd.mld}, we can prove boundedness for
those rationally connected klt Calabi--Yau $3$-folds
that contain an abelian factor.

\begin{cor}\label{t.bdd.ab.cy}
Let $\mathcal{D}_{ab}$ be the set of varieties $X$ such that
\begin{enumerate}
%\item $X$ is a projective klt threefold
\item $X$ is rationally connected klt Calabi--Yau $3$-fold, and
\item $\tilde{q}(X) >0$.
\end{enumerate}
Then $\mathcal{D}_{ab}$ is bounded modulo flops.
\end{cor}

\begin{proof}
%For the reader's convenience we divide the proof into several steps.

{\bf Step 1}. We will construct a quasi-\'etale Galois cover $\gamma:Y\to X=Y/G$ such that $Y$ is either an abelian $3$-fold or a product of an elliptic curve 
and a weak K3 surface (i.e., a normal projective surface $S$ with canonical singularities, $K_S \sim 0$ and $\tilde{q}(S)=0$, cf. \cite{MR2587100}). 


Let $\gamma\colon W_1 \to X$ be the quasi-\'etale
cover given in Theorem \ref{t.ggk}.
Since $\tilde{q}(X) >0$,
it follows that $W_1$ is either an abelian $3$-fold or a product of an elliptic curve 
and a weak K3 surface. Note that $W_1$ has canonical singularities.

%{\bf Step 1}.
%Take 
%\begin{displaymath}
%\xymatrix{
%Y \ar[r] \ar@/_/[rr]_{\gamma} & Z \ar[r]^{\gamma_Z} & X
%}
%\end{displaymath}
%the Stein factorization of $\gamma$.
%As $\gamma$ is quasi\'etale, it follows
%that $Y \to Z$ is a birational map. When $Y$
%is an abelian threefold, then $Y \to Z$ is an isomorphism,
%as $Y$ does not contain any rational curve, see \cite{hm07}.
%In the other case, as $K_Y \sim 0$, it follows that also $K_Z \sim 0$,
%hence $Z$ is canonical. Applying \cite[Proposition 18]{KL}, it follows that
%also $Z \simeq E \times S'$, where $S'$ is a canonical surface with
%$K_{S'} \sim 0$ .
%Hence, up to replacing $Y$ with $Z$ and $\gamma$ with $\gamma_Z$ 
%we can always assume that $\gamma$ is finite.

In view of \cite[Theorem 3.7]{gkp},
there exists a finite surjective morphism $\phi_1 \colon Y_1 \to W_1$
such that $\gamma_1=\gamma\circ  \phi_1$ is Galois and the branch loci of
$\gamma$ and $\gamma_1$ are the same. The latter property implies
that $\gamma_1$ is quasi-\'etale as well as $\phi_1$ is.


If $W_1$ is an abelian $3$-fold, then by purity of the branch locus it 
follows that $\phi_1$ is \'etale and hence  $Y_1$ is also an
abelian $3$-fold. In this case we complete Step 1 by setting $Y=Y_1$.

Now assume that $W_1$ is a product of an elliptic curve 
and a weak K3 surface. Note that $\tilde{q}(W)=1$. 
Now we construct, by induction, a sequence of finite quasi-\'etale surjective morphism
\begin{displaymath}
\xymatrix{
\cdots \ar[r] & Y_i \ar[r]^{\gamma_i} & Y_{i-1} \ar[r]^{\gamma_{i-1}} & \cdots 
\ar[r]^{\gamma_2} & Y_1 \ar[r]^{\gamma_1} &Y_0=X,
}
\end{displaymath} 
such that for each $i$, the compositions $Y_i\to X$ are Galois, and $\gamma_i: Y_i\to Y_{i-1}$ factors as 
\begin{displaymath}
\xymatrix{
Y_i \ar[r]^{\phi_i} & W_{i} \ar[r]^{\psi_{i}} & Y_{i-1},}
\end{displaymath} 
where $W_i$ is a product  of an elliptic curve 
and a weak K3 surface. Moreover, $\psi_i$ is \'etale if $i>1$.

The construction is as the following: assume that we constructed $Y_{i-1}$, then $K_{Y_{i-1}}\sim 0$ and  $Y_{i-1}$ has canonical singularities. By \cite[Theorem 8.3, Corollary 8.4]{Kawamata85}, there exists an \'etale covering $\psi_i: W_{i} \to Y_{i-1}$ where $W_i=C\times Z$, $C$ is an abelian variety and $Z$ is a canonical variety with $K_Z\sim 0$. We only need to show that in our case, $C$ is an elliptic curve and $Z$ is a surface with $\tilde{q}(Z)=0$. Assume not, then it is easy to see that $\tilde{q}{(C\times Z)}>1=\tilde{q}(W_1)$, which is absurd since $\tilde{q}$ is invariant under quasi-\'etale covers.
Then  $\psi_i: W_{i} \to Y_{i-1}$ is constructed by applying  Theorem \ref{t.ggk}, and $\phi_i: Y_i \to W_{i}$ is constructed by applying \cite[Theorem 3.7]{gkp} to the composition $W_i\to X$.
%\begin{enumerate}
%\item[(1)] 
%$\psi_{i}: 
%if $Y_i= E_i \times S_i$ for an elliptic curve $E_i$
%and a canonical surface with $K_{S_i} \sim 0$, then we stop; % and 
%substitute $Y$ with $Y_1$ and $\gamma$ with $\gamma\circ \gamma_1 \circ \dots \gamma_i$;
%\item[(2)] if $Y_i\neq E_i \times S_i$, for an elliptic curve $E_i$
%%and a canonical surface with $K_{S_i} \sim 0$, we use Theorem \ref{t.ggk} and get a map
%$\psi_i\colon F_i \times T_i \to Y_i$. % Using Step 1 we can assume that $\psi_i$ is finite.
%If $\gamma\circ \gamma_1 \circ \dots \gamma_i\circ \psi$ is Galois then we 
%put $Y_{i+1}= F_i \times T_i$ and $\gamma_{i+1} = \psi_i$ and we stop;
%\item[(3)] if $\gamma\circ \gamma_1 \circ \dots \gamma_i\circ \psi$ is not Galois,
%we use Step 2 and we define $Y_{i+1}$ as the Galois closure of the morphism 
%$\gamma\circ \gamma_1 \circ \dots \gamma_i\circ \psi$,
%\begin{displaymath}
%\xymatrix{
%Y_{i+1} \ar[r]^{\phi_i} & F_i \times T_i \ar[r]^{\psi_i} & Y_i \ar[rrr]^{\gamma\circ \gamma_1 \circ \dots \circ  \gamma_i} & & & X,
%}
%\end{displaymath}
%and $\gamma_{i+1} = \psi_i \circ \phi_i$.
%At this point we go back to (1).
%\end{enumerate}

%{\bf Step 3}. %A priori this procedure does not necessarily stop in finite time.
%Let us assume this is the case. 
By \cite[Theorem 1.1]{gkp}, it follows that there exists $i>1$ such 
that $\gamma_i$ is \'etale. %By \cite[Proposition II.8.2.1]{hart} i
It follows that
the morphism $Y_i \to W_i$ is \'etale (see \cite[Corollary 3.6]{milne}). We may write $W_i=E\times S$. As $S$ is simply connected,
 see \cite[Theorem 7.8]{k.shaf}, it follows that $Y_i \simeq E' \times S$ for some
 elliptic curve $E'$. % This shows that the procedure from Step 3 must stop in finite time
 %$n$.
Hence we complete Step 2 by taking $Y=Y_i$.
%Hence, up to replacing $W$ with $Y_i$ and $\gamma$ 
%with the composition $Y_i \to X$, 
%we can assume that $Y$ is either an abelian threefold or a 
%product of an elliptic curve and a weak K3 surface, while $\gamma$ is
%Galois, that is, $X=Y/G$. 

{\bf Step 2}. We will show that the group action of $G$ on $Y$ is bounded.

 As $X=Y/G$ and $Y$ is Gorenstein, if we bound the order 
of the representation of $G$ on the vector space $H^0(Y, K_Y)$ by a universal
constant $C$, then the index of $K_X$ is at most $C!$.
The boundedness modulo flops of $\mathcal{D}_{ab}$ then follows from Theorem \ref{t.bdd.mld}, as the discrepancies of $X$ will all be contained in $\frac{1}{C!} \mathbb{Z}$.
 \iffalse
 is isomorphic to the quotient by the action of a finite
group of automorphisms of $Y$, see \cite[Definition 3.6]{gkp}.
If we can prove that for every $X \in \mathcal{D}_{ab}$ 
the order of $G$ is bounded from above 
by a constant $C \in \mathbb{N}_{>0}$, then the statement of the theorem
follows by Corollary \ref{c.bdd.index}, since $CK_X \sim 0$.
As the group $G$ acts faithfully on $H^0(Y, K_Y) = \mathbb{C}\omega$, 
it is enough to show that for an abelian $3$-fold or a product of an
elliptic curve and a canonical surface with trivial canonical bundle there exists
$C \in \mathbb{N}_{>0}$ such that  if $g$ is an automorphism 
then $g^\ast \omega= \zeta \omega$ where $\zeta$ is a primitive $n$-root
of unity and $n\leq C$.
\fi

{\bf Step 2.1}.
When $Y$ is an abelian $3$-fold, the above claim follows immediately
from the fact that $\mathrm{rk} \;H^3(Y, \mathbb{Z}) = 20$ and for any $g \in G, \; 
g^\ast$ is an automorphism of $H^3(Y, \mathbb{Z})$ defined over the 
integers, hence its minimal polynomial has degree $\leq 20$. That
implies that any eigenvalue of $g^\ast$ is a root of unity of bounded
order. 

{\bf Step 2.2}.
When $Y$ is a product of an elliptic curve $E$ and 
a weak K3 surface $S$ the claim follows in the same vein.
In fact, take $S'\to S$ the minimal resolution, then $S'$ is a K3 surface, and $g$ lifts to an automorphism of $E\times S'$. This
implies that any eigenvalue of $g^\ast$ is a root of unity of bounded
order since $\mathrm{rk} \;H^3(E\times S' , \mathbb{Z}) = 44$.
\iffalse
In fact, as $H^0(Y, K_Y) = H^0(E, K_E) \otimes H^0(S, K_S)$,
it is enough to bound the order of the action of $g^\ast$ given
by an element $g \in G$ on $H^0(E, K_E)$ and $H^0(S, K_S)$
separately. As the projection $Y \to E$ is the Albanese map,
there is a natural action induced by an element 
$g_E \in \mathrm{Aut}(E)$ and the 
minimal polynomial of $g^\ast$ on 
$H^0(E, K_E) = H^1(Y, \Omega^{[1]}_Y)$ has degree at most $2$.
Moreover, we can write $g\colon E\times S \to E \times S$ in the form 
\[
g(e, s) = (g_E(e), g_S(e, s)),
\]
where $g_S \colon E \times S \to S$ is a 
family of automorphisms of $S$ parametrized by $E$.
As the automorphisms of $S$ are discrete, it follows that 
$g_S(e, s)$ does not depend on $E$. Thus,
\[
g(e, s) = (g_E(e), g_S(s)).
\]
The automorphism $g_S$ of $S$ lifts to the minimal 
resolution $S'$ of $S$ and analogously to what we have 
done in Step 2.1, we can bound the mutiplicative order
of the eigenvalues of $g_S^\ast$ on $H^0(S, K_S)
= H^0(S', K_{S'})$ as $\mathrm{rk} \;
H^2(S', \mathbb{Z}) =22$.
\fi
\end{proof}

